GraphMETRO: Mitigating Complex Graph Distribution Shifts via Mixture of Aligned Experts

Graph data are inherently complex and heterogeneous, leading to a high natural diversity of distributional shifts. However, it remains unclear how to build machine learning architectures that generalize to the complex distributional shifts naturally occurring in the real world. Here, we develop GraphMETRO, a Graph Neural Network architecture that models natural diversity and captures complex distributional shifts. GraphMETRO employs a Mixture-of-Experts (MoE) architecture with a gating model and multiple expert models, where each expert model targets a specific distributional shift to produce a referential representation w.r.t. a reference model, and the gating model identifies shift components. Additionally, we design a novel objective that aligns the representations from different expert models to ensure reliable optimization. GraphMETRO achieves state-of-the-art results on four datasets from the GOOD benchmark, which is comprised of complex and natural real-world distribution shifts, improving by 67% and 4.2% on the WebKB and Twitch datasets. Code and data are available at https://github.com/Wuyxin/GraphMETRO.

==> tables/good.tex <==



\begin{table*}[ht]
\setlength{\abovecaptionskip}{0.1cm}
\footnotesize
\centering
% \setlength{\textfloatsep}{3pt}
\resizebox{\textwidth}{!}
{
% \scalebox{0.59}{
% \setlength{\tabcolsep}{0.3mm}{
\begin{tabular}{lllccccccccccccccc}
\toprule[2pt]
\multicolumn{3}{c}{\multirow{3}{*}{covariate}} & \multicolumn{4}{c}{GOOD-HIV\textuparrow} & \multicolumn{4}{c}{GOOD-PCBA\textuparrow} & \multicolumn{4}{c}{GOOD-ZINC\textdownarrow} & \multicolumn{2}{c}{GOOD-CMNIST\textuparrow} & \multirow{11}{*}{graph}\\
\cmidrule(r){4-7} \cmidrule(r){8-11} \cmidrule(r){12-15} \cmidrule(r){16-17}

& & & \multicolumn{2}{c}{scaffold} & \multicolumn{2}{c}{size} & \multicolumn{2}{c}{scaffold} & \multicolumn{2}{c}{size} & \multicolumn{2}{c}{scaffold} & \multicolumn{2}{c}{size} & \multicolumn{2}{c}{color} &\\
\cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11} \cmidrule(r){12-13} \cmidrule(r){14-15} \cmidrule(r){16-17}
& & & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} &\\
\cmidrule(r){1-17}

% & & & \multicolumn{7}{c}{scaffold} & \multicolumn{7}{c}{size}\\
% \cmidrule(r){1-17}
\multicolumn{3}{l}{ERM} & \textbf{82.79} & 69.58 & 83.72  & {59.94} & 33.45 & 16.89 & {34.31} & 17.86 & 0.1224  & {0.1995} & 0.1199 & 0.2427 & 77.96  & 28.60 &\\
\multicolumn{3}{l}{IRM} & 81.35 & 67.97 & 81.33 & 59.00 & 33.56 & 16.90 & 34.28 & \textbf{18.05} & 0.1213 & 0.2025 & 0.1222 & {0.2403} & 77.92 & 27.83 &\\
\multicolumn{3}{l}{VREx} & 82.11 & \textbf{70.77} & 83.47 & 58.53 & \textbf{33.88} & \textbf{16.98} & 34.09 & 17.79 & 0.1211 & 0.2094 & 0.1234 & \textbf{0.2384} & 77.98 & 28.48 &\\
\multicolumn{3}{l}{GroupDRO} & {82.60} & {70.64} & 83.79 & 58.98 & {33.81} & {16.98} & 33.95 & 17.59 & \textbf{0.1168} & \textbf{0.1934} & {0.1180} & 0.2423 & 77.98 & {29.07} &\\
\multicolumn{3}{l}{DANN} & 81.18 & 70.63 & {83.90} & 58.68 & 33.63 & 16.90 & 34.17 & 17.86 & 0.1186 & 0.2004 & 0.1188 & 0.2439 & {78.00} & \textbf{29.14} &\\
\multicolumn{3}{l}{Deep Coral} & 82.53 & 68.61 & \textbf{84.70} & \textbf{60.11} & 33.47 & 16.93 & \textbf{34.49} & {17.94} & {0.1185} & 0.2036 & \textbf{0.1134} & 0.2505 & \textbf{78.64} & 29.05 &\\
\cmidrule(r){1-17}
\multicolumn{3}{l}{Mixup} & 82.29 & 68.88 & 83.16 & 59.03 & 30.22 & 16.59 & 30.63 & 17.06 & 0.1279 & 0.2240 & 0.1255 & 0.2748 & 77.40 & 26.47 &\\
\multicolumn{3}{l}{DIR} & 82.54 & 67.47 & 80.46 & 57.11 & 32.55 & 14.98 & 32.89 & 16.61 & 0.3799 & 0.6493 & 0.1541 & 0.5482 & 31.09 & 20.60 &\\




\midrule[1.5pt]
\multicolumn{3}{c}{\multirow{3}{*}{covariate}} & \multicolumn{4}{c}{GOOD-Motif\textuparrow} & \multicolumn{2}{c}{GOOD-SST2\textuparrow} & & \multicolumn{1}{c}{\multirow{3}{*}{concept}} & \multicolumn{4}{c}{GOOD-Motif\textuparrow} & \multicolumn{2}{c}{GOOD-SST2\textuparrow} & \multirow{11}{*}{graph}\\
\cmidrule(r){4-7} \cmidrule(r){8-9} \cmidrule(r){12-15}\cmidrule(r){16-17}

& & & \multicolumn{2}{c}{base} & \multicolumn{2}{c}{size} & \multicolumn{2}{c}{length} & & & \multicolumn{2}{c}{base} & \multicolumn{2}{c}{size} & \multicolumn{2}{c}{length} &\\
\cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){12-13}\cmidrule(r){14-15}\cmidrule(r){16-17}
& & & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & & & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} &\\
\cmidrule(r){1-9} \cmidrule(r){11-17}

\multicolumn{3}{l}{ERM} & 92.60 & 68.66 & {92.28} & 51.74 & \textbf{89.82} & 81.30 & & \multicolumn{1}{l}{ERM} & {92.02} & {81.44} & {91.73} & \textbf{70.75} & \textbf{94.43} & 72.43 &\\
\multicolumn{3}{l}{IRM} & 92.60 & {70.65} & 92.18 & 51.41 & 89.41 & 79.91 & & \multicolumn{1}{l}{IRM} & 92.00 & 80.71 & 91.68 & 69.77 & 94.10 & \textbf{77.47} &\\
\multicolumn{3}{l}{VREx} & 92.60 & \textbf{71.47} & 92.25 & \textbf{52.67} & 89.51 & 80.64 & & \multicolumn{1}{l}{VREx} & \textbf{92.05} & \textbf{81.56} & 91.67 & 70.24 & 94.26 & 73.16 &\\
\multicolumn{3}{l}{GroupDRO} & {92.61} & 68.24 & \textbf{92.29} & {51.95} & 89.59 & \textbf{81.35} & & \multicolumn{1}{l}{GroupDRO} & 92.01 & 81.43 & 91.67 & 69.98 & 94.41 & 71.86 &\\
\multicolumn{3}{l}{DANN} & 92.60 & 65.47 & 92.23 & 51.46 & 89.60 & 79.71 & & \multicolumn{1}{l}{DANN} & {92.02} & 81.33 & \textbf{91.81} & {70.72} & 94.02 & 76.03 &\\
\multicolumn{3}{l}{Deep Coral} & {92.61} & 68.88 & 92.22 & 50.97 & 89.68 & 79.81 & & \multicolumn{1}{l}{Deep Coral} & 92.01 & 81.37 & 91.68 & 70.49 & 94.25 & 72.34 &\\
\cmidrule(r){1-9} \cmidrule(r){11-17}
\multicolumn{3}{l}{Mixup} & \textbf{92.68} & 70.08 & 92.02 & 51.48 & 89.78 & 80.88 & & \multicolumn{1}{l}{Mixup} & 91.89 & 77.63 & 91.45 & 67.81 & 94.12 & 73.34 &\\
\multicolumn{3}{l}{DIR} & 87.73 & {61.50} & 84.53 & 50.41 & 84.30 & 77.65 & & \multicolumn{1}{l}{DIR} & 91.60 & 72.14 & 73.10 & 56.28 & 93.71 & 68.76 &\\


\midrule[1.5pt]
\multicolumn{3}{c}{\multirow{3}{*}{concept}} & \multicolumn{4}{c}{GOOD-HIV\textuparrow} & \multicolumn{4}{c}{GOOD-PCBA\textuparrow} & \multicolumn{4}{c}{GOOD-ZINC\textdownarrow} & \multicolumn{2}{c}{GOOD-CMNIST\textuparrow} & \multirow{11}{*}{graph}\\
\cmidrule(r){4-7} \cmidrule(r){8-11} \cmidrule(r){12-15} \cmidrule(r){16-17}

& & & \multicolumn{2}{c}{scaffold} & \multicolumn{2}{c}{size} & \multicolumn{2}{c}{scaffold} & \multicolumn{2}{c}{size} & \multicolumn{2}{c}{scaffold} & \multicolumn{2}{c}{size} & \multicolumn{2}{c}{color}  &\\
\cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11} \cmidrule(r){12-13} \cmidrule(r){14-15} \cmidrule(r){16-17}
& & & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}}  &\\
\cmidrule(r){1-17}

\multicolumn{3}{l}{ERM} & {84.22} & 72.33 & 88.05 & 63.26 & 25.95 & 21.63 & 32.54 & 15.36 & 0.1222 & 0.1306 & 0.1315 & 0.1403 & 90.00 & 42.87  &\\
\multicolumn{3}{l}{IRM} & 82.89 & 72.59 & \textbf{88.62} & 59.90 & 25.89 & 21.22 & {32.99} & {16.07} & 0.1225 & 0.1314 & 0.1278 & {0.1368} & {90.02} & 42.80  &\\
\multicolumn{3}{l}{VREx} & 83.84 & 72.60 & {88.28} & 60.23 & \textbf{26.62} & {22.02} & 32.49 & 15.59 & {0.1186} & {0.1270} & 0.1309 & 0.1419 & 89.99 & {43.31}  &\\
\multicolumn{3}{l}{GroupDRO} & 83.40 & \textbf{73.64} & {88.28} & 61.37 & 26.32 & 21.83 & \textbf{33.03} & 15.99 & 0.1207 & 0.1281 & \textbf{0.1251} & 0.1369 & \textbf{90.02} & \textbf{43.32}  &\\
\multicolumn{3}{l}{DANN} & 83.87 & 71.92 & 87.28 & {65.27} & 26.07 & 21.64 & 32.74 & 15.78 & \textbf{0.1172} & \textbf{0.1256} & {0.1253} & \textbf{0.1339} & 89.94 & 43.11  &\\
\multicolumn{3}{l}{Deep Coral} & \textbf{84.65} & {72.97} & 87.88 & 62.28 & {26.38} & {21.95} & 32.67 & {16.20} & 0.1187 & 0.1279 & 0.1287 & 0.1370 & 89.94 & 43.16  &\\
\cmidrule(r){1-17}
\multicolumn{3}{l}{Mixup} & 82.36 & 72.03 & 87.64 & {64.87} & 23.73 & 19.78 & 30.23 & 13.36 & 0.1353 & 0.1475 & 0.1423 & 0.1522 & 89.95 & 40.96  &\\
\multicolumn{3}{l}{DIR} & 83.28 & 69.05 & 79.19 & \textbf{72.61} & 25.85 & \textbf{22.20} & 30.53 & \textbf{16.86} & 0.3501 & 0.3865 & 0.2348 & 0.2871 & 86.76 & 22.69  &\\


\midrule[1pt]
\midrule[1pt]
\multicolumn{3}{c}{\multirow{3}{*}{covariate}} & \multicolumn{4}{c}{GOOD-Cora\textuparrow} & \multicolumn{4}{c}{GOOD-Arxiv\textuparrow} & \multicolumn{2}{c}{GOOD-CBAS\textuparrow} & \multicolumn{2}{c}{GOOD-Twitch\textuparrow} & \multicolumn{2}{c}{GOOD-WebKB\textuparrow} & \multirow{11}{*}{node}\\
\cmidrule(r){4-7} \cmidrule(r){8-11} \cmidrule(r){12-13} \cmidrule(r){14-15} \cmidrule(r){16-17}

& & & \multicolumn{2}{c}{word} & \multicolumn{2}{c}{degree} & \multicolumn{2}{c}{time} & \multicolumn{2}{c}{degree} & \multicolumn{2}{c}{color} & \multicolumn{2}{c}{language} & \multicolumn{2}{c}{university}  &\\
\cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11} \cmidrule(r){12-13} \cmidrule(r){14-15} \cmidrule(r){16-17}
& & & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}}  &\\
\cmidrule(r){1-17}

\multicolumn{3}{l}{ERM} & 70.43 & {64.86} & 72.27 & 56.30 & {72.69} & 71.08 & 77.47 & 58.91 & 89.29 & 76.00 & 70.66 & 48.95 & 38.25 & 14.29 &\\
\multicolumn{3}{l}{IRM} & 70.27 & 64.77 & {72.64} & 56.28 & 72.66 & 71.04 & 77.50 & 58.98 & 91.00 & 76.00 & 69.75 & 47.21 & 39.34 & 13.49 &\\
\multicolumn{3}{l}{VREx} & 70.47 & 64.80 & 72.25 & 56.30 & 72.66 & 71.12 & 77.49 & 58.99 & \textbf{91.14} & 77.14 & 70.66 & 48.99 & 39.34 & 14.29 &\\
\multicolumn{3}{l}{GroupDRO} & 70.41 & 64.72 & 72.18 & 56.29 & 72.68 & {71.15} & 77.46 & \textbf{59.08} & 90.86 & 76.14 & 70.84 & 47.20 & 39.89 & 17.20 &\\
\multicolumn{3}{l}{DANN} & {70.66} & 64.77 & 72.47 & 56.10 & \textbf{72.74} & 71.05 & {77.51} & {59.00} & 90.14 & \textbf{77.57} & 70.67 & 48.98 & 39.89 & 15.08 &\\
\multicolumn{3}{l}{Deep Coral} & 70.47 & 64.72 & 72.16 & {56.35} & 72.66 & 71.07 & 77.48 & 58.97 & \textbf{91.14} & 75.86 & 70.67 & 49.64 & 38.25 & 13.76 &\\
\cmidrule(r){1-17}
\multicolumn{3}{l}{Mixup} & \textbf{71.54} & \textbf{65.23} & \textbf{74.57} & \textbf{58.20} & 72.49 & \textbf{71.34} & \textbf{77.61} & 57.60 & 73.57 & 70.57 & 71.30 & \textbf{52.27} & \textbf{54.65} & 17.46 &\\
\multicolumn{3}{l}{EERM} & 68.79 & 61.98 & 73.32 & 56.88 & OOM & OOM & OOM & OOM & 67.62 & 52.86 & \textbf{73.87} & 51.34 & 46.99 & \textbf{24.61} &\\
\multicolumn{3}{l}{SRGNN} & 70.27 & 64.66 & 71.37 & 54.78 & 72.50 & 70.83 & 75.96 & 57.52 & 77.62 & 74.29 & 70.58 & 47.30 & 39.89 & 13.23 &\\

\midrule[1.5pt]
\multicolumn{3}{c}{\multirow{3}{*}{concept}} & \multicolumn{4}{c}{GOOD-Cora\textuparrow} & \multicolumn{4}{c}{GOOD-Arxiv\textuparrow} & \multicolumn{2}{c}{GOOD-CBAS\textuparrow} & \multicolumn{2}{c}{GOOD-Twitch\textuparrow} & \multicolumn{2}{c}{GOOD-WebKB\textuparrow} & \multirow{11}{*}{node}\\
\cmidrule(r){4-7} \cmidrule(r){8-11} \cmidrule(r){12-13} \cmidrule(r){14-15} \cmidrule(r){16-17}

& & & \multicolumn{2}{c}{word} & \multicolumn{2}{c}{degree} & \multicolumn{2}{c}{time} & \multicolumn{2}{c}{degree} & \multicolumn{2}{c}{color} & \multicolumn{2}{c}{language} & \multicolumn{2}{c}{university}  &\\
\cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11} \cmidrule(r){12-13} \cmidrule(r){14-15} \cmidrule(r){16-17}
& & & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}} & \multicolumn{1}{c}{ID\textsubscript{ID}} & \multicolumn{1}{c}{OOD\textsubscript{OOD}}  &\\
\cmidrule(r){1-17}
\multicolumn{3}{l}{ERM} & 66.05 & {64.60} & {68.71} & 60.54 & 74.76 & 67.32 & \textbf{75.27} & {62.99} & 89.79 & 82.36 & 80.29 & 57.32 & 65.00 & 27.83 &\\
\multicolumn{3}{l}{IRM} & 66.09 & {64.60} & 68.58 & {61.23} & 74.67 & 67.41 & 75.23 & 62.97 & 90.71 & \textbf{83.21} & 77.05 & 59.17 & 65.56 & 27.52 &\\
\multicolumn{3}{l}{VREx} & 66.00 & 64.57 & 68.45 & 60.58 & {74.80} & 67.37 & 75.19 & \textbf{63.00} & 89.50 & 82.86 & 80.29 & 57.37 & 65.00 & 27.83 &\\
\multicolumn{3}{l}{GroupDRO} & {66.17} & \textbf{64.62} & 68.37 & 60.65 & 74.73 & \textbf{67.45} & 75.19 & 62.88 & 90.36 & 82.00 & 81.95 & \textbf{60.27} & 65.00 & 28.14 &\\
\multicolumn{3}{l}{DANN} & 66.16 & 64.51 & 68.08 & 60.78 & 74.73 & 67.28 & {75.25} & 62.91 & 89.93 & 82.50 & 80.28 & 57.46 & 65.00 & 26.91 &\\
\multicolumn{3}{l}{Deep Coral} & 66.13 & 64.58 & 68.38 & 60.58 & 74.77 & {67.42} & 75.16 & 62.85 & 89.36 & 82.64 & 80.14 & 56.97 & 65.00 & 28.75 &\\
\cmidrule(r){1-17}
\multicolumn{3}{l}{Mixup} & \textbf{69.66} & 64.44 & \textbf{70.32} & \textbf{63.65} & \textbf{74.92} & 64.84 & 72.75 & 61.28 & \textbf{93.64} & 64.57 & 78.89 & 55.28 & \textbf{67.22} & \textbf{31.19} &\\
\multicolumn{3}{l}{EERM} & 65.75 & 63.09 & 66.50 & 58.38 & OOM & OOM & OOM & OOM & 78.33 & 64.29 & \textbf{83.91} & 51.94 & 61.67 & 27.83 &\\
\multicolumn{3}{l}{SRGNN} & 66.45 & \textbf{64.62} & 68.34 & 61.08 & 74.64 & 67.17 & 74.83 & 62.09 & 88.57 & 81.43 & 80.21 & 56.05 & 61.67 & 27.52 &\\

\bottomrule[2pt]
\end{tabular}
}
\vspace{0.4cm}
% }
\caption{}
\label{table:real}
\end{table*}
